Stylistic Attribute Control in Latent Diffusion Models

Text-to-image diffusion models have revolutionized image synthesis and editing, but precise control over stylistic attributes remains a challenge, often causing unintended content modifications. We propose an approach for fine-grained parametric control of stylistic attributes in latent diffusion models by learning disentangled editing directions from synthetic datasets. We use guidance composition to close the domain gap between stylistically finetuned and foundation models, preserving the original image semantics while applying stylistic adjustments. To ensure consistent edits, we introduce a training regularization loss and enhance DDIM inversion with optimized null-conditional embeddings for real image editing. We validate our approach by learning from stylistically filtered synthetic datasets varying a range of stylistic attributes, including outlines, local contrast, watercolorization effects, and geometric patterns. Our evaluations demonstrate that compared to current text-based editing techniques, our method offers well-integrated, more precise and continuously adjustable stylistic modifications.

==> background.tex <==
\section{Background} %
\label{sec:background}

Diffusion models progressively add random noise to input data through a variance-preserving Markov process~\cite{sohl2015deep,ho2020denoising,song2020score}. They then learn to reverse this process by denoising, thereby generating the desired data samples. Latent Diffusion Models~\cite{rombach2022high} apply this process in a low-dimensional latent space $z$, where a Variational Autoencoder (VAE)~\cite{kingma2013auto} first encodes an image $I$ into $z_0 = \mathcal{E}(I)$ using a pretrained encoder $\mathcal{E}(\cdot)$ and then noise is added to $z_0$ for $t=1...T$ timesteps until $z_T\sim \mathcal{N}(0,I)$.
During the denoising phase, the model predicts the noise delta $\varepsilon_{\theta}(z_t,t,c)$ at each timestep $t$, moving from $z_t$ to $z_{t-1}$. Here, $\varepsilon_{\theta}$ is a neural network, often a U-Net~\cite{ronneberger2015u}, and $c$ represents conditioning information, in our case text embeddings $c_{\text{p}}$. The training loss in text-to-image models \cite{rombach2022high} minimizes the difference between the actual noise $\varepsilon \sim \mathcal{N}(0,I)$ and the predicted noise $\varepsilon_{\theta}$:
\begin{equation}
\label{eq:diffusion_loss}
L = \mathbb{E}_{\mathcal{E}(I), c_{\text{p}},\varepsilon,t}\left[\lVert \varepsilon-\varepsilon_{\theta}(z_t, t, c_{\text{p}}) \rVert_{2}^{2} \right], t=1,...,T
\end{equation}
After the model is trained, it can effectively denoise from $z_T$ back to $z_0$ using an efficient diffusion sampler~\cite{song2020denoising, lu2022dpm}. 
Finally, the decoded image $I$ is reconstructed using a frozen decoder $\mathcal{D}(\cdot)$.
The model is trained concurrently on both conditional ($c$) and unconditional (null-text embedding $\emptyset$) objectives. During inference, the difference between unconditioned and (text) conditioned outputs, denoted as vector $\Vec{g_p}$, can guide the generative process towards the conditioned goal. This classifier-free guidance (CfG)~\cite{hojonathanClassifierFreeDiffusionGuidance2022} is computed as
\begin{align}
\Vec{g_p} &= \varepsilon_{\theta}(z_t,t, c_{\text{p}}) - \varepsilon_{\theta}(z_t,t,\emptyset) \\
 \varepsilon_{\theta}(z_t,t,g_p) &= \varepsilon_{\theta}(z_t,t,\emptyset) + wg_p
\label{eq:cfg}
\end{align}
where, $w$ is the CfG scale that adjusts the intensity of the guidance. %










